Uncertainty Aware System Identification with Universal Policies

Sim2real transfer is primarily concerned with transferring policies trained in simulation to potentially noisy real world environments. A common problem associated with sim2real transfer is estimating the real-world environmental parameters to ground the simulated environment to. Although existing methods such as Domain Randomisation (DR) can produce robust policies by sampling from a distribution of parameters during training, there is no established method for identifying the parameters of the corresponding distribution for a given real-world setting. In this work, we propose Uncertainty-aware policy search (UncAPS), where we use Universal Policy Network (UPN) to store simulation-trained task-specific policies across the full range of environmental parameters and then subsequently employ robust Bayesian optimisation to craft robust policies for the given environment by combining relevant UPN policies in a DR like fashion. Such policy-driven grounding is expected to be more efficient as it estimates only task-relevant sets of parameters. Further, we also account for the estimation uncertainties in the search process to produce policies that are robust against both aleatoric and epistemic uncertainties. We empirically evaluate our approach in a range of noisy, continuous control environments, and show its improved performance compared to competing baselines.

==> abstract.tex <==
In sim2real reinforcement learning it is essential to learn policies that are robust to real-world noises. Often, an associated problem with sim2real is to estimate the real-world environmental parameters to ground the simulated environment. Domain Randomisation (DR), by using a distribution of parameters during training, can produce robust policies. But there is no proper method to identify the parameters of the corresponding distribution for a given real-world setting. In this work, we use Universal Policy Network (UPN) to store simulation-learnt task-specific policies across the full range of environmental parameters and then subsequently employ robust Bayesian optimisation to craft robust policies for the given environment by combining relevant UPN policies in a DR like fashion. Such policy-driven grounding is known to be more efficient as it estimates only task-relevant sets of parameters. Further, we also account for the estimation uncertainties in the search process to produce policies that are robust against both aleatoric and epistemic uncertainties. We empirically evaluate our approach in a range of noisy, continuous control environments, and show its improved performance compared to the baselines.


\begin{comment}

Learning policies that are robust to real-world noises is an essential requirement for deploying reinforcement learning agents on real-world tasks. Although recent attempts using domain randomisation have shown to produce robust policies, they suffer from over randomisation that can produce over generalised policies. In contrast, matching exact parameters of real-world tasks can produce high performing, but low robust policies. In this work, we propose to use a Universal Policy Networks based parameter estimation workflow that integrates the uncertainty caused by the noise in real-world and the model bias, in its parameter estimations and policy construction. We empirically evaluate our approach in a range of continuous control environments, and show its improved performance compared to the baselines.

\end{comment}

